Human-Modeling in Sequential Decision-Making: An Analysis through the Lens of Human-Aware AI

"Human-aware" has become a popular keyword used to describe a particular class of AI systems that are designed to work and interact with humans. While there exists a surprising level of consistency among the works that use the label human-aware, the term itself mostly remains poorly understood. In this work, we retroactively try to provide an account of what constitutes a human-aware AI system. We see that human-aware AI is a design oriented paradigm, one that focuses on the need for modeling the humans it may interact with. Additionally, we see that this paradigm offers us intuitive dimensions to understand and categorize the kinds of interactions these systems might have with humans. We show the pedagogical value of these dimensions by using them as a tool to understand and review the current landscape of work related to human-AI systems that purport some form of human modeling. To fit the scope of a workshop paper, we specifically narrowed our review to papers that deal with sequential decision-making and were published in a major AI conference in the last three years. Our analysis helps identify the space of potential research problems that are currently being overlooked. We perform additional analysis on the degree to which these works make explicit reference to results from social science and whether they actually perform user-studies to validate their systems. We also provide an accounting of the various AI methods used by these works.

==> SarathSections/2-method-new.tex <==
\textcolor{red}{Over the past decade, there has been a growing interest in understanding how to effectively integrate the human-in-the-loop. This trend is evident in the growing number of related papers at major AI conferences. This shift stems from the recognition that AI operates in human environments, necessitating systems that understand and adapt to human behaviors. 
This evolution reflects a move towards a more interdisciplinary approach in AI, integrating cognitive science, psychology, and social sciences \cite{miller2019explanation}, and encouraging human-centered methods in the design of AI systems \cite{chetouani2023humancentred}.
This has also led to a veritable explosion in the number of works that try to introduce AI methods that can help with improving human-AI interaction.
Given the constraints of a workshop paper, we can't realistically carry out an exhaustive review of all the relevant papers. 
}
